Partially Conditioned Patch Parallelism for Accelerated Diffusion Model Inference

Diffusion models have exhibited exciting capabilities in generating images and are also very promising for video creation. However, the inference speed of diffusion models is limited by the slow sampling process, restricting its use cases. The sequential denoising steps required for generating a single sample could take tens or hundreds of iterations and thus have become a significant bottleneck. This limitation is more salient for applications that are interactive in nature or require small latency. To address this challenge, we propose Partially Conditioned Patch Parallelism (PCPP) to accelerate the inference of high-resolution diffusion models. Using the fact that the difference between the images in adjacent diffusion steps is nearly zero, Patch Parallelism (PP) leverages multiple GPUs communicating asynchronously to compute patches of an image in multiple computing devices based on the entire image (all patches) in the previous diffusion step. PCPP develops PP to reduce computation in inference by conditioning only on parts of the neighboring patches in each diffusion step, which also decreases communication among computing devices. As a result, PCPP decreases the communication cost by around $70\%$ compared to DistriFusion (the state of the art implementation of PP) and achieves $2.36\sim 8.02\times$ inference speed-up using $4\sim 8$ GPUs compared to $2.32\sim 6.71\times$ achieved by DistriFusion depending on the computing device configuration and resolution of generation at the cost of a possible decrease in image quality. PCPP demonstrates the potential to strike a favorable trade-off, enabling high-quality image generation with substantially reduced latency.

==> tables/eval-record.tex <==
4 gpus 0.3 partial

1024
ours: Latency: 2.13441 s 2.13515
their: Latency: 2.16447 s 

2048
ours: Latency: 6.68500 s
theirs: Latency: 7.14246 s
41
3440
ours: 23.95
theirs: Latency: 28.25392 s

3648
ours: 27.76320
theirs: 32.92


8 gpus 0.8 partial

1024
ours: Latency: 1.64663 s
theirs: Latency: 1.67834 s

2048
ours: Latency: 4.13632 s
theirs: Latency: 4.43830 s

3840
ours: Latency: 17.46744 s
theirs: 20.86


image quality 

